Self-supervised Learning with Local Contrastive Loss for Detection and Semantic Segmentation

We present a self-supervised learning (SSL) method suitable for semi-global tasks such as object detection and semantic segmentation. We enforce local consistency between self-learned features, representing corresponding image locations of transformed versions of the same image, by minimizing a pixel-level local contrastive (LC) loss during training. LC-loss can be added to existing self-supervised learning methods with minimal overhead. We evaluate our SSL approach on two downstream tasks -- object detection and semantic segmentation, using COCO, PASCAL VOC, and CityScapes datasets. Our method outperforms the existing state-of-the-art SSL approaches by 1.9% on COCO object detection, 1.4% on PASCAL VOC detection, and 0.6% on CityScapes segmentation.

==> Main/1_introduction.tex <==
% \vspace{-2mm}
\section{Introduction}

% no one cites the fukushima paper for SSL -- so I don't know why we are doing that?
% \cite{fukushima1980neocognitron}.


Self-supervised learning (SSL) approaches are capable of learning generic feature representations from data in the absence of any external supervision. In computer vision, a common strategy adopted by SSL approaches is to apply multiple transformations to an image and then requiring that the features extracted from the different transformed copies must be similar \cite{chen2020simplesimclr,he2020momentummoco}. \sudipta{Isn't this called contrastive loss? who were amongst the first to propose it?}
SSL in vision remains an active area of research~\cite{caron2020unsupervisedswav,caron2021emergingdino,grill2020bootstrapbyol,he2020momentummoco}.
Recently proposed SSL methods have shown great promise. Training a simple image classifier using logistic regression, that takes the features learned via SSL as input and predicts the image category \cite{chen2020simplesimclr,he2020momentummoco,grill2020bootstrapbyol}.
BYOL~\cite{grill2020bootstrapbyol} and SwaV~\cite{caron2020unsupervisedswav} are examples of SSL methods that are used to train ResNet50 features~\cite{he2016deepresnet} that achieved 74.3\% and 75.3\% top-1 accuracy on ImageNet whereas the top-1 accuracy achieved by training ResNet50 features in a fully supervised setting is 76.6\%.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/teaser_new.png}
    % \vspace{-2.4mm}
    \caption{\small Existing self-supervised learning approaches typically do not impose local consistency during training. Given an image and its transformed copy, these methods learn features by encouraging the global features from both images to be similar. We propose a new loss that encourages local regions in the two images to also produce similar features.\sudipta{Figure and caption needs work -- we know other methods also impose local consistency constraints. Furthermore we say 'we propose a new loss that' but the figure is not neither explaining what the new loss function is or why it is new. The red circles, crosses and white lines must be explained.}}
    % \vspace{-4mm}
    % \sudipta{make figures side-by-side.}
    %The corresponding pairs are automatically obtained via data augmentation.
    \label{fig:teaser}
\end{figure}

The loss functions used by existing SSL methods to train convolutional neural network or vision transformer \cite{DBLP:conf/iclr/DosovitskiyB0WZ21} backbones are well suited for learning global features that are suitable for the image categorization task. However, such representations do not retail spatial information which makes them less suitable for semi-global tasks such as object detection, instance segmentation and semantic segmentation.

Recent work has tried to address the above-mentioned issue by extending contrastive loss functions used in SSL to incorporate additional correspondence constraints in the transformed copies of the same image. In these existing approaches, the correspondence constraints are enforced either over coarse image regions\cite{wei2021aligningsoco,xiao2021regionresim} or at a dense and fine-grained pixel level~\cite{wang2021densecl,xie2021propagatepixpro}. We argue that neither of these two strategies explored in previous work achieve exact locality that is easily attained from image transformation.\sudipta{The previous two sentences are crucial because we are pointing out what is lacking in previous approaches such as SoCo, DenseCL, PixPro. However, whatever we are saying in the current version is not convincing.} \ash{Yes, this sentence needs to be changed. I will edit it. Moreover, SoCo actually uses the image transformation based locality.}
To address the aforementioned limitation, we propose a new loss function that we refer to as Local Correspondence Loss (\putalg). The main idea in \putalg is that \textcolor{red}{[fill in the blanks]}. Say that \putalg can be used alongwith the conventional global contrastive losses. This is different from DenseCL and PixPro because \textcolor{red}{[fill in the blank]}.
Figure \ref{fig:teaser} illustrates the basic idea.\sudipta{current figure is not illustrating much, use it to emphasize the difference with DenseCL and, or PixPro. Can we show three cartoon figures side-by-side, to emphasize what how the three different methods impose correspondence constraints?}. 
We output a peaked probability distribution over corresponding locations and perform maximum likelihood estimation over that probability distribution.\sudipta{what probability distribution? what is max likelihood estimation being used to estimate?}
Note that true pixel correspondences are known since the input image pairs used in self-supervised approaches are generated by applying two distinct transformations to a single image. 
We evaluate the impact of using LC-loss on several downstream tasks, namely object detection, instance segmentation and semantic segmentation and report promising improvements over previous SSL methods on Pascal VOC, COCO, Cityscapes and ScanNet datasets.


%\textcolor{red}{Many computer vision tasks are inherently spatial in nature. Spatially localized (local) feature representations are arguably more important than global representations for tasks such as semantic segmentation, image correspondences and object detection. Previous works that incorporate local sensitivity in self-supervised learning either employ region based correspondences \cite{wei2021aligningsoco,xiao2021regionresim} or use the learned dense representations \cite{wang2021densecl,xie2021propagatepixpro} to find the best correspondences. We argue that either of the two constraints misses exact locality that is easily attained from image transformation. We propose a Local Correspondence Loss (\putalg)  that explicitly considers both local and global representations during training. Figure \ref{fig:teaser} illustrates the basic idea. In addition to the objective of making the global feature representations similar for the two images, \putalg imposes local consistency between corresponding regions of image pairs obtained from transformations of the same image. Since CNNs and ViTs inherently produce spatial features, \putalg can be used alongside any self-supervised learning method with minimum computational overhead. We output a peaked probability distribution over corresponding locations and perform maximum likelihood estimation over that probability distribution. Note that true pixel correspondences are known since the input image pairs used in self-supervised approaches are generated by applying two distinct transformations to a single image. We empirically verify that our LC-loss approach results in superior representations for detection and segmentation tasks.}

We note that our \putalg is inspired from local feature matching methods from geometric vision literature. The idea of local consistency between transformed versions of the same image for self-supervised learning has been also done before (See Sec.~\ref{sec:literature}). Our novelty lies not in the individual components or algorithms, but in the full methodology. We apply ideas of local feature matching from geometric vision, and use a simple maximum likelihood estimation over corresponding local features to estimate a local loss function that can be easily incorporated to an existing self-supervised learning framework.\sudipta{this paragraph is very vague.}

\customparagraph{Contributions.} Our LCL work includes the following key technical contributions: \textbf{(1)} a novel local correspondence loss (\putalg) method that performs maximum likelihood estimation over the probability distribution of corresponding pixels of two augmented versions of the same image, that can be added to any self-supervised learning method, such as BYOL; and \textbf{(2)} state-of-the-art transfer learning results for BYOL in several dense labeling tasks. Using ResNet-50 backbones pretrained on ImageNet, our BYOL variant outperforms the BYOL baseline by {\bf 4.3\%} AP and {\bf 2.9\%} mIoU for PASCAL VOC object detection and segmentation, {\bf 1.9\%} AP for COCO object detection, {\bf 1.9\%} mIoU for CityScapes segmentation, and {\bf 3.2\%} mIoU for ScanNet segmentation.
\sudipta{in the previous paragraph, we use the phrase "dense labeling tasks" which we have not defined yet. replace it with something else which does not need to be explained.}

% \begin{comment}
% After generating corresponding pairs, the next question is how to apply local loss function. One potential solution is to use the similar loss function for dense correspondence as the global loss function. For example, DenseCL \cite{wang2021densecl} uses contrastive loss for both local and global consistency. However, we propose a loss function that is agnostic to the self-supervised framework. 

% There are very few works that perform self-supervised learning at pixel-level representations \cite{wang2021densecl, xie2021propagatepixcontrast}. Both DenseCL \cite{wang2021densecl} and PixContrast \cite{xie2021propagatepixcontrast} aim to generate corresponding pairs between local feature representations of two augmented versions of the same image, and then apply local loss on the corresponding pairs. To generate proper correspondence, they calculate similarity between all local feature pairs and pick the pairs with maximum similarity. This framework suffers from a chicken and egg issue, where the similarity function will be sub-optimal before learning good feature representations, and to learn a good feature representations the loss function has to be optimized that requires measuring similarity between features. We argue that it's possible to select corresponding pixels from the image augmentation. 
% \end{comment}

==> Main/5_experiments.tex <==
\section{Experimental Results}

We evaluate object detection and segmentation performance on the PASCAL VOC \cite{everingham2010pascalvoc}, MS COCO \cite{lin2014microsoftcoco}, CityScapes \cite{cordts2016cityscapes}, and ScanNet \cite{dai2017scannet} datasets. We perform two experiments - `finetuning' and `frozen'. In funetuning, we finetune all the layers including the pretrained backbone. We also report detection and segmentation results for frozen backbone following \cite{xiao2021regionresim,henaff2021efficientdetcon,goyal2019scalinggoyal}. Training a linear classifier on a frozen backbone is a standard approach to evaluate self-supervised representation quality for image classification \cite{he2020momentummoco,chen2020bigsimclrv2,grill2020bootstrapbyol,caron2020unsupervisedswav}. We also adopt the same strategy in `frozen backbone' setting, i.e., where we freeze the pretrained ResNet50 backbone and only finetune the remaining layers. Frozen backbone might be an ideal evaluation strategy for because finetuning the full network evaluates quality of representations along with initialization and optimization, whereas frozen backbone evaluates mostly the representation quality of the backbone \cite{goyal2019scalinggoyal,xiao2021regionresim}. In the following, we report the main results.


\begin{table*}[!htbp]
    \centering
    \caption{\small \textbf{Main Results.} We use faster-RCNN with RetinaNet for COCO object detection,  Mask-RCNN with FPN for COCO instance segmentation, faster RCNN with FPN for VOC object detection. In `finetuned' setting, we finetune all the layers including the pretrained backbone, and in `frozen' setting, we freeze the pretrained backbone and only finetune the remaining layers.\ben{Which of these are published results and which are trained from published checkpoints?}}
    \label{tab:main_results}
    \begin{subtable}{\textwidth}
        \centering
        \caption{\bf Finetuned Backbone}
        \label{tab:main_ft}
        \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{l c | c c c | c c c| c c c}
                \toprule
                \multirow{4}{*}{\bf \small Method}      & {}                    & \multicolumn{6}{c|}{\small \bf COCO}         & \multicolumn{3}{c}{\bf \small PASCAL VOC}                                                                                                                                                                      \\
                                                        & {}                    & \multicolumn{3}{c|}{\small Object Detection} & \multicolumn{3}{c|}{\small Instance Segmentation} & \multicolumn{3}{c}{Object Detection}                                                                                                                       \\
                                                        & {\bf \small Pretrain} & \multicolumn{3}{c|}{\small RetinaNet + FPN}  & \multicolumn{3}{c|}{\small Mask-RCNN + FPN}       & \multicolumn{3}{c}{{ \small FRCNN + FPN}}                                                                                                                  \\
                                                        & {\bf \small Epochs}   & { $\text{AP}^b$}                             & { $\text{AP}^b_{50}$}                             & { $\text{AP}^b_{75}$}                     & AP$^{mk}$  & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & { $\text{AP}^b$} & { $\text{AP}^b_{50}$} & {$\text{AP}^b_{75}$} \\
                \midrule
                % Scratch                                    & -                     & -                                           & -                                           & -                                        & -           & -           & -    & 32.8              & 59.0                   & 31.6                      \\
                Supervised  \cite{he2016deepresnet}     & 90                    & 37.7                                         & 57.2                                              & 40.4                                      & 35.4       & 56.5           & 38.1           & 53.2             & 81.7                  & 58.2                 %& 55.4              & 82.1                   & 60.9                      \\
                \\
                Moco v2   \cite{chen2020improvedmocov2} & 200                   & 37.3                                         & 56.2                                              & 40.4                                      & 36.4       & 57.2           & 38.9           & 55.6             & 81.3                  & 61.8                 \\
                BYOL  \cite{grill2020bootstrapbyol}     & 300                   & 35.4                                         & 54.7                                              & 37.4                                      & 37.2       & 58.8           & 39.8           & 55.0             & 83.1                  & 61.1
                %& 56.9              & 83.4                   & 64.2               \\
                \\
                \midrule
                DetCo        \cite{xie2021detco}        & 800                   & 38.4                                         & 57.8                                              & 41.2                                      & 36.4       & 58.0           & 38.9           & 56.7             & 82.3                  & 63.0                 \\
                ReSim-FPN \cite{xiao2021regionresim}    & 200                   & 38.6                                         & 57.6                                              & 41.6                                      & 36.0       & 57.1           & 38.6           & 57.8             & 82.7                  & 65.4                 \\
                SCRL \cite{roh2021spatiallyscrl}        & 800                   & 39.0                                         & 58.7                                              & 41.9                                      & 37.7       & 59.6           & 40.7           & 57.2             & 83.8                  & 63.9                 \\
                SoCo    \cite{wei2021aligningsoco}      & 400                   & 38.3                                         & 57.2                                              & 41.2                                      & 38.2       & {\bf 60.2}     & {41.0}         & 57.4             & 82.6                  & 64.7                 \\
                \midrule
                DenseCL       \cite{wang2021densecl}    & 200                   & 37.6                                         & 56.6                                              & 40.2                                      & 36.4       & 57.0           & 39.2           & 56.6             & 81.8                  & 62.9                 \\
                PixPro   \cite{xie2021propagatepixpro}  & 400                   & 38.7                                         & 57.5                                              & 41.6                                      & -          & -              & -              & 58.7             & 82.9                  & 65.9                 \\
                \rowcolor{_teal3} \ours                 & 400                   & \bf40.6                                      & \bf60.4                                           & \bf43.6                                   & {\bf 38.3} & {60.0}         & {\bf 41.1}     & \bf60.1          & \bf84.2               & \bf67.8              \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{subtable}
    % Frozen
    \begin{subtable}{\textwidth}
        \centering
        \caption{\bf Frozen Backbone}
        \label{tab:main_frozen}
        \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{l c | c c c | c c c| c c c}
                \toprule
                \multirow{4}{*}{\bf \small Method}      & {}                    & \multicolumn{6}{c|}{\small \bf COCO}         & \multicolumn{3}{c}{\bf \small PASCAL VOC}                                                                                                                                                                     \\
                                                        & {}                    & \multicolumn{3}{c|}{\small Object Detection} & \multicolumn{3}{c|}{\small Instance Segmentation} & \multicolumn{3}{c}{Object Detection}                                                                                                                      \\
                                                        & {\bf \small Pretrain} & \multicolumn{3}{c|}{\small Retina-FPN}       & \multicolumn{3}{c|}{\small Mask-RCNN + FPN}       & \multicolumn{3}{c}{{ \small FRCNN + FPN}}                                                                                                                 \\
                                                        & {\bf \small Epochs}   & { $\text{AP}^b$}                             & { $\text{AP}^b_{50}$}                             & { $\text{AP}^b_{75}$}                     & AP$^{mk}$ & AP$^{mk}_{50}$ & AP$^{mk}_{75}$ & { $\text{AP}^b$} & { $\text{AP}^b_{50}$} & {$\text{AP}^b_{75}$} \\
                \midrule
                Supervised  \cite{he2016deepresnet}     & 90                    & 30.3                                         & 50.0                                              & 31.3                                      & 31.5      & 51.4           & 33.4           & 50.7             & 80.4                  & 55.1

                \\
                Moco v2   \cite{chen2020improvedmocov2} & 200                   & 28.0                                         & 46.3                                              & 29.1                                      & 31.4      & 51.2           & 33.3           & 52.7             & 80.9                  & 57.6                 \\
                BYOL  \cite{grill2020bootstrapbyol}     & 300                   & 30.2                                         & 49.1                                              & 31.5                                      & 31.7      & 51.4           & 33.7           & 52.4             & 81.1                  & 57.5                 \\
                \midrule
                DetCo        \cite{xie2021detco}        & 800                   & 27.6                                         & 45.9                                              & 28.5                                      & 31.1      & 50.7           & 33.0           & 51.3             & 79.9                  & 56.5                 \\
                ReSim-FPN \cite{xiao2021regionresim}    & 200                   & 27.7                                         & 45.4                                              & 29.0                                      & 32.2      & 51.7           & 34.4           & 53.7             & 81.4                  & 59.6                 \\
                SoCo    \cite{wei2021aligningsoco}      & 400                   & 28.9                                         & 46.8                                              & 30.4                                      & 30.9      & 50.7           & 32.8           & 52.0             & 80.0                  & 56.4                 \\
                \midrule
                DenseCL       \cite{wang2021densecl}    & 200                   & 25.5                                         & 43.6                                              & 25.8                                      & 30.9      & 50.8           & 32.5           & 50.9             & 79.9                  & 55.0                 \\
                PixPro   \cite{xie2021propagatepixpro}  & 400                   & 27.7                                         & 44.6                                              & 29.1                                      & 31.1      & 50.5           & 33.2           & 53.5             & 80.4                  & 59.7                 \\
                \rowcolor{_teal3} \ours                 & 400                   & \bf30.5                                      & \bf49.8                                           & \bf31.7                                   & \bf33.3   & \bf53.6        & \bf35.6        &
                \bf55.1                                 & \bf82.6               & \bf61.7                                                                                                                                                                                                                                                      \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{subtable}


\end{table*}



\subsection{Object Detection and Instance Segmentation}

% \sudipta{Reorganize all the text in this subsection into three paragraphs.}

In the following, we show object detection and segmentation results on downstream COCO and PASCAL VOC dataset.  We use detectron2 framework \cite{wu2019detectron2} for evaluation.

\customparagraph{COCO Object Detection.}
For object detection on COCO, we adopt RetinaNet \cite{lin2017focalretina} network following \cite{wei2021aligningsoco,roh2021spatiallyscrl,xie2021detco}. We finetune all layers with Sync BatchNorm for 90k iterations on COCO \texttt{train2017} set and evaluate on COCO \texttt{val2017} set. Table \ref{tab:main_ft} shows object detection results on COCO for our method and other approaches in the literature with full-network finetuning. Note that ReSim, SoCo, and SCRL use region proposal networks during pretraining on ImageNet, hence, these approaches are not exactly comparable to ours. Our model is more similar with methods like DetCo, DenseCL, and PixPro. We achieve 40.6 AP for object detection tasks outperforming the second best method PixPro \cite{xie2021propagatepixpro} by a significant 1.9\%. We outperform the baseline BYOL by a huge margin of 5.1\% AP. For frozen backbone, we achieve 30.5\% AP outperforming PixPro by 2.8\% AP.


% Talk about results specific to COCO object detection. refer to Table~\ref{tab:coco_mrcnn} and discuss both frozen backbone and finetued backbone.

\customparagraph{PASCAL VOC Object Detection.}
We report object detection results for PASCAL VOC \cite{everingham2010pascalvoc}. We use the Faster-RCNN \cite{ren2016fasterrcnn} object detector with ResNet50-FPN backbone following \cite{roh2021spatiallyscrl}. For training, we use images from both \texttt{trainval07+12} sets and we evaluate only on the VOC07 \texttt{test07} set. We use the pretrained checkpoints released by the authors for the backbone network, and finetune on the VOC dataset. Table \ref{tab:main_results} shows that we achieve 60.1 AP for VOC detection in finetuning setting. Our method improves mean AP by a significant 3.2\% over baseline BYOL, and outperform the current SOTA PixPro by 1.4\% AP. The improvement is even more significant in AP75, where we outperform BYOL by 3.6\% and PixPro by 1.9\%. For frozen setting (Table \ref{tab:main_frozen}), we acheive 55.1\% AP for VOC detection, outperforming PixPro by 1.6\% and BYOL by 2.7\%.

\customparagraph{COCO Instance Segmentation.}
For instance segmentation on COCO, we use Mask-RCNN framework \cite{he2017maskrcnn} with the ResNet50-FPN backbone. We follow the $1\times$ schedule. Table \ref{tab:main_ft} reports the instance segmentation performance on COCO. Our method achieves 38.3\% AP for COCO instance segmentation, which is comparable with the SoCo \cite{wei2021aligningsoco}. Note that SoCo performs selective search on the input image to find object proposals, and uses additional feature pyramid networks during pretraining, whereas our pretraining setting is much simpler. Table \ref{tab:main_frozen}  shows  significant improvement in frozen backbone setting. Our method acheive 33.3\% AP with frozen backbone for COCO instance segmentation, outperforming PixPro by 1.2\% and SoCo by 1.4\% AP. Note that Mask-RCNN also outputs object detection results that are reported in the Appendix.

\subsection{Semantic Segmentation}
We show semantic segmentation evaluation in Table \ref{tab:main_segm} on PASCAL VOC, CityScapes \cite{cordts2016cityscapes}, and ScanNet \cite{dai2017scannet} datasets for both finetuning and frozen backbone setting. We use FCN backbone \cite{long2015fullyfcn} following the settings in \texttt{mmsegmentation} \cite{mmseg2020}.

\customparagraph{PASCAL VOC Segmentation.}
% \sudipta{Talk about relevant results. refer to Table~\ref{tab:coco_mrcnn} and discuss both frozen backbone and finetued backbone.}
For PASCAL VOC segmentation, we train on  VOC \texttt{train-aug2012} set for 20k
iterations and evaluate on val2012 set. Table \ref{tab:segm_ft} reports mIoU results for segmentation on the VOC2007 test set. Our method yields 72.1\% mIoU outperforming BYOL by a 7.7\% and PixPro by 1\% mIoU. For frozen backbone setting, we achieve 63.4\% mIoU, which is \textit{more than the score achieved by BYOL in finetuning setting (63.3\% mIoU)}. We also outperform PixPro by a significant 2.9\% mIoU.

\customparagraph{Cityscapes Segmentation.}
CityScapes \cite{cordts2016cityscapes} contain images from urban street scenes. Table \ref{tab:segm_ft} shows that for finetuning setting our approach yield 77.8\% AP which is 6.2\% mIoU improvement over BYOL and 0.6\% improvement over PixPro. In frozen backbone setting (Table \ref{tab:segm_frozen}), we achieve 60.7\% mIoU which improves upon BYOL by 5.1\% and PixPro by 2.5\%.

\customparagraph{ScanNet Segmentation.}
ScanNet is a dataset of RGB-D scans of real world environments from 1513 scans acquired in 707 distinct spaces; hence the dataset contains images from indoor scenes. We sample $\sim$20k images from 1201 scans as the training set and $\sim$5.5k images from 312 scans as the test set for semantic segmentation. On ScanNet, we achieve 55.5\% mIoU outperforming BYOL by 7.2\% mIoU and PixPro by 2.5\% mIoU in finetuning setting. In frozen setting, our method outperform BYOL by 6.4\% achieving 37.4\% mIoU.

% \sudipta{Please split up the text into two paragraphs, one for Cityscapes and one for ScanNet.}
% CityScapes \cite{cordts2016cityscapes} and ScanNet \cite{dai2017scannet} are very different from the PASCAL VOC and COCO datasets. On the other hand, CityScapes contain images from urban street scenes. Table \ref{tab:city_scane} reports semantic segmentation performance for both the CityScapes and ScanNet datasets. For both datasets, we use a FCN ResNet50-C4 network and finetune the network for 40k iterations. On CityScapes, our method achieves 6.2\% mIoU improvement over BYOL. On ScanNet, we outperform BYOL by 7.2\% mIoU. We achieve state-of-the-art performance for both datasets.



\begin{table}[!htbp]
    \centering
    \caption{\small Evaluation on Semantic Segmentation using FCN ResNet-50 network.}
    \label{tab:main_segm}
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{Finetuning}
        \label{tab:segm_ft}
        \begin{tabular}{l  c | c | c | c}
            \toprule
            \multirow{2}{*}{\bf Method} & {\bf Pretrain} & {\bf VOC}      & {\bf CityScapes} & {\bf ScanNet}
            \\
                                        & {Epochs}       & {mIoU}         & {mIoU}           & {mIoU}        \\
            \midrule
            % Scratch             & 53.9       \\
            Scratch                     & -              & 40.7           & 63.5             & 44.1          \\
            %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
            %  \midrule
            Supervised                  & 90             & 67.7           & 74.6             & 52.4          \\ %68.2       \\
            Moco v2                     & 200            & 67.5           & 74.5             & 53.4          \\ %68.9       \\
            BYOL                        & 300            & 63.3           & 71.6             & 48.3          \\ % 64.4       \\
            \midrule
            DetCo                       & 800            & 70.1           & 75.7             & 54.3          \\
            ReSim                       & 200            & \boldsec{72.1} & 77.4             & 54.6          \\
            SoCo                        & 400            & 70.0           & 75.2             & 52.2          \\
            \midrule
            DenseCL                     & 200            & 69.4           & 69.4             & 54.8          \\
            PixPro                      & 400            & 71.1           & 77.2             & 54.6          \\
            \rowcolor{_teal3} \ours     & 400            & \bf72.1        & \bf77.8          & \bf55.5       \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \hspace{.05\textwidth}
    % Frozen
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{Frozen}
        \label{tab:segm_frozen}
        \begin{tabular}{ c | c | c}
            \toprule
            {\bf VOC}                 & {\bf CityScapes} & {\bf ScanNet}
            \\
            {mIoU}                    & {mIoU}           & {mIoU}        \\
            \midrule
            % Scratch             & 53.9       \\
            -                         & -                & -             \\
            %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
            %  \midrule
            56.6                      & 55.7             & 32.2          \\
            58.3                      & 59.1             & 33.4          \\
            55.7                      & 55.6             & 31.0          \\
            \midrule
            56.1                      & 57.2             & 29.1          \\
            61.2                      & 58.1             & 36.3          \\
            55.2                      & 56.7             & 30.0          \\
            \midrule
            63.0                      & 58.8             & 36.0          \\
            60.3                      & 58.2             & \bf37.4       \\
            \rowcolor{_teal3} \bf63.4 & \bf60.7          & \bf37.4       \\
            \bottomrule
        \end{tabular}
    \end{subtable}
\end{table}


% \begin{table}[!htbp]
%     \centering
%     \caption{{\small {\bf Object detection and semantic segmentation on PASCAL VOC with R50-FPN and FCN backbone respectively.}}}
%     % \vspace{-3mm}
%     \label{tab:pascal}
%     \begin{subtable}[t]{0.55\textwidth}
%         \centering
%         \caption{VOC Object Detection}
%         \label{tab:pascal_det}
%         \begin{tabular}{p{0.35\linewidth} c  c  c  c}
%             \toprule
%             {\bf Method}            & {\bf $\text{AP}$} & {\bf $\text{AP}_{50}$} & {\bf $\text{AP}_{75}$} \\
%             \midrule
%             Scratch                 & 32.8              & 59.0                   & 31.6                   \\
%             %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
%             %  \midrule
%             Supervised              & 55.4              & 82.1                   & 60.9                   \\
%             Moco v2                 & 55.6              & 81.3                   & 61.8                   \\
%             BYOL                    & 56.9              & 83.4                   & 64.2                   \\
%             \midrule
%             DetCo                   & 56.7              & 82.3                   & 63.0                   \\
%             ReSim                   & 57.8              & 82.7                   & 65.4                   \\
%             SoCo                    & 57.4              & 82.6                   & 64.7                   \\
%             \midrule
%             DenseCL                 & 56.6              & 81.8                   & 62.9                   \\
%             PixPro                  & 58.7              & 82.9                   & 65.9                   \\
%             \rowcolor{_teal3} \ours & \bf60.1           & \bf84.2                & \bf67.8                \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}
%     \hspace{0.01\textwidth}
%     \begin{subtable}[t]{0.4\textwidth}
%         \centering
%         \caption{VOC Semantic Segmentation}
%         \label{tab:pascal_segm}
%         \begin{tabular}{p{0.35\linewidth}  c  c  c  c}
%             \toprule
%             {\bf Method}            & {\bf mIoU}     \\
%             \midrule
%             % Scratch             & 53.9       \\
%             Scratch                 & 40.7           \\
%             %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
%             %  \midrule
%             Supervised              & 67.7           \\ %68.2       \\
%             Moco v2                 & 67.5           \\ %68.9       \\
%             BYOL                    & 63.3           \\ % 64.4       \\
%             \midrule
%             DetCo                   & 70.1           \\
%             ReSim                   & \boldsec{72.1} \\
%             SoCo                    & 70.0           \\
%             \midrule
%             DenseCL                 & 69.4           \\
%             PixPro                  & 71.1           \\
%             \rowcolor{_teal3} \ours & \bf72.1        \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}
% \end{table}


% \begin{table}[!htbp]
%     \centering
%     \begin{adjustbox}{max width=\linewidth}
%         \begin{tabular}{l c  c  c  c}
%             \toprule
%                                       & \multicolumn{3}{c}{\bf\small Detection} & \multicolumn{1}{c}{\bf\small Segm}                                         \\
%             \cmidrule(lr){2-4} \cmidrule(lr){5-5}
%             {\bf Method}               & {\bf $\text{AP}^b$}                     & {\bf $\text{AP}^b_{50}$}           & {\bf $\text{AP}^b_{75}$} & {\bf mIoU} \\
%             \midrule
%             Scratch                    & 32.8                                    & 59.0                               & 31.6                     & 53.9       \\
%             %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
%             %  \midrule
%             Supervised IN *            & 54.2                                    & 81.6                               & 59.8                     & 67.7       \\
%             BYOL IN *                  & 51.9                                    & 81.0                               & 56.5                     & 63.3       \\
%             BYOL IN                    & 51.0                                    & 80.6                               & 55.5                     & 68.6       \\
%             \rowcolor{_teal3} \ours IN & 55.3                                    & 82.7                               & 62.5                     & 71.5       \\
%             \midrule
%             %  MoCo-v2 CC & 54.7 & 81.0 & 60.6 & 64.5 \\
%             MoCo-v2 CC                 & 53.8                                    & 80.4                               & 59.6                     & 65.1       \\
%             BYOL CC                    & 54.4                                    & 80.6                               & 60.5                     & 66.9       \\
%             \rowcolor{_teal3} \ours CC & 57.1                                    & 81.7                               & 63.4                     & 68.9       \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
%     \caption{{\small {\bf Object detection and semantic segmentation on PASCAL VOC.} `IN' and 'CC' refer to ImageNet and COCO pretrained models, respectively. (*) denotes pretrained models from official or third-party implementations \cite{wang2021densecl}.}}
%     % \vspace{-3mm}
%     \label{tab:pascal}
% \end{table}



% \begin{table}[!htbp]
%     \centering
%     \caption{\small {\bf CityScapes and ScanNet Segmentation.}}
%     % \caption{{\small {\bf Segmentation on CityScapes and ScanNet.} We finetune the pretrained backbones for 40k iterations with FCN ResNet50-C4 network. For CityScapes, our method achieves 1.9\% mIoU improvement over BYOL for ImageNet pretrained backbone and 1.7\% improvement for COCO pretrained backbone. For ScanNet, we outperform BYOL by 3.2\% for ImageNet pretrained and 1.8\% mIoU for COCO pretrained backbone.\todo{Remove commentary as it is already in the main text.} }}
%     % \vspace{-3mm}
%     \label{tab:city_scane}
%     \begin{subtable}[t]{0.45\textwidth}
%         \centering
%         \caption{CityScapes Segmentation}
%         \begin{tabular}{l c }
%             \toprule
%             {\bf Method}            & {\bf CityScapes} \\
%             \midrule
%             Scratch                 & 63.5             \\
%             Supervised              & 74.6             \\
%             Moco v2                 & 74.5             \\
%             BYOL                    & 71.6             \\
%             \midrule
%             DetCo                   & 75.7             \\
%             ReSim                   & 77.4             \\
%             SoCo                    & 75.2             \\
%             \midrule
%             DenseCL                 & 69.4             \\
%             PixPro                  & 77.2             \\
%             \rowcolor{_teal3} \ours & \bf77.8          \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}
%     \begin{subtable}[t]{0.45\textwidth}
%         \centering
%         \caption{ScanNet Segmentation}
%         \begin{tabular}{l c }
%             \toprule
%             {\bf Method}            & {\bf ScanNet} \\
%             \midrule
%             Scratch                 & 44.1          \\
%             Supervised              & 52.4          \\
%             Moco v2                 & 53.4          \\
%             BYOL                    & 48.3          \\
%             \midrule
%             DetCo                   & 54.3          \\
%             ReSim                   & 54.6          \\
%             SoCo                    & 52.2          \\
%             \midrule
%             DenseCL                 & 54.8          \\
%             PixPro                  & 54.6          \\
%             \rowcolor{_teal3} \ours & \bf55.5       \\
%             \bottomrule
%         \end{tabular}
%     \end{subtable}
%     % \end{adjustbox}
%     % \vspace{-2mm}
% \end{table}





% \todo{Semantic segmentation on ScanNet with ScanNet-pretrained models}

% \ash{Should we discuss more on ScanNet pretraining, as most of our ablations and analysis during internship were performed on ScanNet?}

% \subsection{Results on CityScapes}
% \todo{Semantic segmentation on CityScapes}



% \subsection{Frozen Backbone}
% \sudipta{Remove this sub section. Discuss the frozen backbone results where they are presented in tables in earlier subsections.}
% % \todo{Show results for frozen backbone finetuning}
% In frozen backbone evaluation, we freeze the ResNet-50 backbone network and only finetune the RPN, FPN or classifier networks. This can be an ideal evaluation for representation learning for object detection or semantic segmentation, as with freezing the backbone we are not evaluating the initialization or optimization methods for finetuning the full backbone \cite{goyal2019scaling}. Table \ref{tab:frozen} shows the results for frozen backbone on VOC object detection with faster-RCNN w/ FPN, COCO object detection Mask-RCNN w/ FPN, VOC segmentation with FCN, and CityScapes segmentation with FCN network. We use the pretrained backbone checkpoints released by the authors, and finetune the remaining layers using detectron2 \cite{wu2019detectron2} framework. Our method outperforms all the other approaches.


% \subsection{Comparison on Image Classification}


==> Main/6_ablation.tex <==
\section{Analysis}


\customparagraph{Efficient Pre-training.}
% \todo{Show results for smaller image-size and epoch, and show that our method can outperform even 100 epoch BYOL model}
In table \ref{tab:efficient}, we report results of VOC object detection with fasterRCNN-FPN, COCO object detection from MaskRCNN-FPN, VOC and CityScapes segmentation from FCN for BYOL and \ours pretrained with different epochs. Results reveal that \textit{our model pretrained with 200 epochs and with training image-size 160 can achieve better results than BYOL pretrained with 1000 epochs saving 5.3$\times$ computational resource}. Even our 100-epoch-pretrained model seems to be comparable with 1000-epoch-pretrained BYOL model. \textit{This validates efficacy of our local local loss during self-supervised pretraining}.

\begin{table*}[!htbp]
    \centering
    \caption{\small \textbf{Efficient Pre-training on ImageNet.} We show performance on object detection and segmentation for BYOL and \ours for different pretraining epochs and training image-size. We achieve better performance than BYOL (1000 epochs pretraining) with our model pretrained with 200 epochs and with training image-size 160 that is 5.3$\times$ faster to pretrain.}
    \label{tab:efficient}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l c c | c | c | c | c | c}
            \toprule
            \multirow{2}{*}{\bf \small Method} & {\bf \small Pretrain} & {\bf \small Pretrain} & {\bf \small Pretrain} & \multicolumn{1}{c|}{{\bf \small VOC}} & \multicolumn{1}{c|}{\bf \small COCO} & {\bf \small VOC} & {\bf \small Cityscapes} \\
                                               & {\bf \small Epochs}   & {\bf \small Im-size}  & {\bf \small time}     & { $\text{AP}^b$}                      & { $\text{AP}^b$}                     & {mIoU}           & {mIoU}                  \\
            \midrule

            BYOL                               & 300                   & 224                   & $\times$1.6           & 56.9                                  & 40.4                                 & 63.3             & 71.6                    \\
            BYOL                               & 1000                  & 224                   & $\times$5.3           & 57.0                                  & 40.9                                 & 69.0             & 73.4                    \\
            \midrule
            \ours                              & 100                   & 224                   & $\times$0.8           & 58.2                                  & 40.9                                 & 68.4             & 76.5                    \\
            \ours                              & 200                   & 160                   & $\times$1             & 59.0                                  & 41.6                                 & 68.5             & 77.0                    \\
            \ours                              & 200                   & 224                   & $\times$1.6           & 59.6                                  & 42.0                                 & 70.9             & 77.4                    \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}





\customparagraph{Importance of Local Contrast}
% \ben{I think this paragraph should be called something like: ``The importance of local contrast''. We have a great opportunity to point out that global BYOL works better than global contrastive loss, but that local BYOL is much worse than Local Contrastive loss. Why is that? We need to see the standard arguments for BYOL vs. Contrastive and understand why they don't apply \emph{locally}. I think this would be more interesting than the ``DencseCL-like'' or ``max'' variants.}
In Table \ref{tab:other_corr}, we perform experiments where we change our local contrastive loss to non-contrastive BYOL-type loss function. In, \ours (BYOL-like), we apply the same L2-normalized MSE loss function in the local loss as the global loss in BYOL. All the models are trained for 800 epochs on the COCO dataset, and results for ImageNet pretrained models are reported in the Appendix. We report the average AP scores for PASCAL VOC in Table \ref{tab:other_corr}, which shows that our approach of calculating local  consistency using contrastive loss works better than non-contrastive BYOL-type local loss.
\begin{table}[!htbp]
    \centering
    \begin{minipage}[r]{0.4\textwidth}
        \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{c|c}
                \toprule
                {\small \bf Method} & {\small \bf VOC (AP)} \\
                \midrule
                BYOL                & 54.81                 \\
                % \ours (Random) & - \\
                \ours (BYOL-like)   & 55.98                 \\
                % \ours (DenseCL-like) & 55.85                 \\
                % \ours (max)          & 54.91                 \\
                \ours               & {\bf 57.22}           \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}
    \hspace{0.01\textwidth}
    \begin{minipage}[l]{0.5\textwidth}
        \caption{{\small The effect of different variations of local loss function. Results are reported in terms of average AP for PASCAL VOC object detection with the faster-RCNN framework.}}
        \label{tab:other_corr}
    \end{minipage}
\end{table}

\customparagraph{Few-shot Image Classification.}
Since global and local losses appear to be complementary to each other, we ask whether our method hurts the image classification performance for transfer learning in various datasets. For this experiment, we use our pretrained models as fixed feature extractors, and perform 5-way 5-shot few-shot learning on 7 datasets from diverse domains using a logistic regression classifier. Table \ref{tab:fshot} report the 5-shot top-1 accuracy for the EuroSAT \cite{helber2019eurosat}, CropDisease \cite{mohanty2016cropdisease}, ChestX \cite{wang2017chestx}, Sketch \cite{wang2019learningsketch}, ISIC \cite{codella2019skinisic}, Sketch \cite{wang2019learningsketch}, DTD \cite{cimpoi2014describingdtd}, and Omniglot \cite{lake2015humanomniglot} datasets. Table \ref{tab:fshot} reveals that \ours show best performance on average among the self-supervised models that use local consistency. For example, it outperforms PixPro by 2.4\% top-1 accuracy on average the minor fluctuation can be attributed to random noise.


\begin{table*}[!htbp]
    % \vspace{-1mm}
    \centering
    \caption{{\small {\bf Few-shot learning results on downstream datasets.} The pretrained models are used as fixed feature extractors We report top-1 accuracy for 5-way 5-shot averaged over 600 episodes. We use the publicly available pretrained backbone as feature extractor for the few-shot evaluation.}\ben{Again- are these published results or our own?} \ash{Our results}}
    % \vspace{-2mm}
    \label{tab:fshot}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{c|c c c c c c c | c}
            \toprule
            {\bf Method} & {\bf EuroSAT} & {\bf CropDisease} & {\bf ChestX} & {\bf ISIC} & {\bf Sketch} & {\bf DTD} & {\bf Omniglot} & {\bf Avg} \\
            \midrule
            % BYOL CC      & 80.9          & 91.6              & 27.1         & 80.2         & 90.2           & 83.4           & 75.6      \\
            % \ours CC     & 83.5          & 90.9              & 26.5         & 81.1         & 91.2           & 82.0           & 75.9      \\
            % \midrule
            % BYOL         \\
            Supervised   & 85.8          & 92.5              & 25.2         & 43.4       & 86.3         & 81.9      & 93.0           & 72.6      \\
            \midrule
            SoCo         & 78.3          & 84.1              & 25.1         & 41.2       & 81.5         & 73.9      & 92.2           & 68.0      \\
            DenseCL      & 77.7          & 81.0              & 23.8         & 36.8       & 76.5         & 78.3      & 77.4           & 64.5      \\
            PixPro       & 80.5          & 86.4              & 26.5         & 41.2       & 81.5         & 73.9      & 92.2           & 68.9      \\
            \ours        & 84.5          & 90.1              & 25.2         & 41.9       & 85.6         & 80.2      & 91.5           & 71.3      \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    % \vspace{-2.6mm}
\end{table*}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{example-image-a}
%     \caption{Experiments on COCO-pretrained models.}
%     \label{fig:my_label}
% \end{figure}

% \customparagraph{Computational Complexity.}
% \ben{This is pretty weak as is and, without more information and comparison, should probably be dropped. Let's get a proper quantitative measure for ``complexity'' and talk about that instead.}Our \putalg has minimum overhead over the BYOL for the training time. To train our network for 200 epochs, it takes around 31 hour 30 min, whereas without the \putalg it takes 31 hour 17 min. Hence, it is just 1\% slower than BYOL. 

\section{Ablation Studies} \label{sec:ablation}

\customparagraph{Effect of Pretraining Epochs.}
Figure \ref{fig:abl_ep} reports object detection performance on PASCAL VOC with faster-RCNN-FPN and MSCOCO with Mask-RCNN-FPN for different numbers of pretraining epochs. The models are pretrained on the ImageNet training set. Longer training generally results in better downstream object detection performance. For example, for the 100 epoch pretrained model, the AP is 39.8\%, whereas for the 600 epoch pretrained model it improves to 42.8\% for COCO evaluation. The same can be observed for PASCAL VOC object detection.

% \begin{figure}[!htbp]
%     % \vspace{-2mm}
%     \centering
%     \begin{minipage}[c]{0.6\textwidth}
%     \includegraphics[width=0.45\linewidth]{Figures/abl_ep_coco.png}
%     \includegraphics[width=0.45\linewidth]{Figures/abl_ep_pascal.png}    
%     \end{minipage}
%     \begin{minipage}[c]{0.3\textwidth}
%     \caption{{\bf \small Effect of longer training.} The plot shows average AP for object detection on PASCAL VOC (left) and COCO validation sets (right). The models were pretrained on the COCO dataset.}
%     % \vspace{-3mm}
%     \label{fig:abl_ep}
%     \end{minipage}
% \end{figure}


\begin{figure}[!htbp]
    % \vspace{-2mm}
    \centering
    \begin{subfigure}{0.55\textwidth}
        \centering
        \includegraphics[width=0.45\linewidth]{Figures/abl_ep_coco.png}
        \includegraphics[width=0.45\linewidth]{Figures/abl_ep_pascal.png}
        \caption{{\bf \small Effect of longer pre-training.} The plot shows average AP for object detection on COCO validation sets (left) and PASCAL VOC (right).}
        \label{fig:abl_ep}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{Figures/abl_nre.png}
        \caption{{\bf \small Effect of relative weights of \putalg}. The plot shows the average AP for object detection on VOC.}
        \label{fig:abl_alpha}
    \end{subfigure}
\end{figure}





\customparagraph{Ablation on Loss Weight $\alpha$.}
% \ben{Can we offer better anaylsis than this? Clearly the numbers suggest that a balance between global and local losses gets the best local performance. Can we do anything more in depth here?}
Figure \ref{fig:abl_alpha} reports the performance for object detection on PASCAL VOC in terms of average AP for different values of the weight parameter $\alpha$. The models are pretrained on the ImageNet dataset for 200 epochs with training image-size of 160 for faster training. $\alpha$ balances the weight between the global and local loss functions. For $\alpha=0.05$, the mean AP is 58.4\%. We get a slightly better performance with $\alpha=0.1$ (58.9\%) and $\alpha=0.3$ (59.0\%). The performance degrades a little when $\alpha$ is increased to $\alpha=0.7$ (57.5\%). Results reveal the best performance is achieved when we use both global and local loss functions, and a proper balance between them ensure better downstream performance.

% \subsection{Correspondence loss with Multi-scale feature}
% \todo{Ablation on grid-size: Add an upsampling decoder and then try ours. Or, use multi-scale features to measure correspondence loss.}

% \subsection{Effect of data augmentation}
% \ash{Should we do this? depends on timing.}

% \todo{Show qualitative example for correspondence - multi-scale}
% \todo{Failure cases - show pictures}

% \section{Qualitative Examples}
% \todo{Can't these two sections be subsections of ``Analysis"? It saves us the section header...}

% \begin{figure*}[!tbp]
%     \centering
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/2_0000_o.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/5_0000_o_coco.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/3_0002_o.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/10_0002_o.jpg}
%     \\
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/2_0000_p_corr.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/5_0000_corr_coco.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/3_0002_p_corr.jpg}
%     \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/10_0002_p_corr.jpg}
%     \caption{{\small }}
%     \label{fig:my_label}
% \end{figure*}

\section{Qualitative Analysis}
\customparagraph{Correspondence Visualization.}
In Figure \ref{fig:vis_corr}, we show some visual examples of correspondence from our model. For two transformed images $I_1$ and $I_2$, we extract feature representations $F_1$ and $F_2$. For each feature in $F_1$, the corresponding feature in $F_2$ is calculated based on maximum cosine similarity between the feature representations. We show the matching at the original image resolution. Figure \ref{fig:vis_corr} shows that our method predicts accurate matches most of the time (considering the resolution error due to the $32\times 32$ grid size in the pixel space for each feature point).

\begin{figure}[!tbp]
    \centering
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/2_0000_o.jpg}
    % \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/5_0000_o_coco.jpg}
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/3_0002_o.jpg}
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/10_0002_o.jpg}
    \\
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/2_0000_p_corr.jpg}
    % \includegraphics[width=0.24\linewidth]{Figures/store_plot_corr/5_0000_corr_coco.jpg}
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/3_0002_p_corr.jpg}
    \includegraphics[width=0.32\linewidth]{Figures/store_plot_corr/10_0002_p_corr.jpg}
    % \vspace{-2mm}
    \caption{{\small {\bf Correspondence Visualization.} (Top) Ground-truth correspondence between two transformed versions of the same image. (Bottom) Correspondence prediction from \ours. }}
    % \vspace{-4mm}
    \label{fig:vis_corr}
\end{figure}


\customparagraph{More Analysis on Correspondence.}
To show that our method is learning better correspondence across datasets, we perform a simple experiment. Given an image, we flip the image along the horizontal direction, and apply color transformations (Gaussian blur, color-jitter, and random grayscale operations). Since the only spatial transformation is horizontal flipping, the corresponding pixels are simply at the mirror locations of the original pixels, i.e., for a pixel location (x,y), the correct correspondence location in the transformed image is (w-x, y), where w is the width. Note that the correspondence is measured in the feature locations, not in actual pixel locations. We can also measure the correspondence accuracy based on whether the matching is correct or not. We use the ImageNet pretrained backbone from BYOL and \ours, and evaluate the correspondence on the COCO dataset. Figure \ref{fig:more_corr} shows some visual examples of the correspondence map on images from the COCO dataset. We also measure the accuracy of correct correspondences on the COCO val dataset. For the BYOL pretrained model, the accuracy is only $\sim$33\%, PixPro achieves $\sim$99\% accuracy, and \ours achieves $\sim$96\% accuracy. The results suggest that our approach is more robust against color transformations. We infer that PixPro achieves better accuracy as PixPro is trained only with local consistency loss, whereas we use both global and local correspondence during pretraining. The models have not been trained on COCO. Hence, the results also show that the correspondence maps generalize to other datasets.

\begin{figure}[!tbp]
    \centering
    % \begin{subfigure}[c]{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0000_o.jpg}
    %     \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0008_o.jpg}
    %     \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0026_o.jpg}
    %     \caption{GT}
    % \end{subfigure}
    \begin{subfigure}[c]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0000_byol.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0008_byol.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0026_byol.jpg}
        \caption{BYOL}
    \end{subfigure}
    \begin{subfigure}[c]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0000_pix.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0008_pix.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0026_pix.jpg}
        \caption{PixPro}
    \end{subfigure}
    \begin{subfigure}[c]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0000_ours.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0008_ours.jpg}
        \includegraphics[width=0.95\linewidth]{Figures/store_plt_sym/0_0026_ours.jpg}
        \caption{\ours}
    \end{subfigure}
    \caption{\small {\bf Correspondence map for an image and its transformed versions with only flipping and color transformation.} (a) Results from BYOL without local loss. There are many erroneous corresponding pixels denoting that global loss alone does not learn good features for local correspondence. (b) and (c): Results from PixPro and \ours, both of which perfectly detects most of the correspondences.}
    % \vspace{-3.5mm}
    \label{fig:more_corr}
\end{figure}

% \begin{figure}[!tbp]
%     \centering

%     % \vspace{-3mm}
%     \begin{minipage}[c]{0.6\textwidth}
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/9_0003_wo.jpg}
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/9_0003_corr_coco.jpg} \\
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/11_0005_wo.jpg}
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/11_0005_corr_coco.jpg} \\
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/14_0002_wo.jpg}
%         \includegraphics[width=0.44\linewidth]{Figures/store_sym/14_0002_corr_coco.jpg} \\
%     \end{minipage}
%     % \vspace{-2mm}
%     \begin{minipage}[c]{0.35\textwidth}
%         \caption{{\small Correspondence map for an image and its transformed versions with only flipping and color transformation. (Left) Results from BYOL without local loss. There are many erroneous corresponding pixels denoting that global loss alone does not learn good features for local correspondence. (Right) Results from \ours, which perfectly detects most of the correspondences.}\ben{We should also visualize results from pixpro}}
%         % \vspace{-3.5mm}
%         \label{fig:more_corr}
%     \end{minipage}
% \end{figure}


==> Main/backup.tex <==

\todo{Put finetune and frozen together....}

\begin{table*}[!htbp]
    \centering
    \caption{\small \textbf{Frozen backbone evaluation.} We freeze the ResNet-50 backbone and finetune the other layers (RPN, FPN, classifier networks, regression layers, etc.). We use faster-RCNN with FPN for PASCAL VOC object detection, Mask-RCNN with FPN for COCO detection, and FCN network for VOC and CityScapes segmentation.}
    \label{tab:frozen}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{p{0.16\linewidth} | c c c | c c c| c | c}
            \toprule
            \multirow{2}{*}{\bf \small Method} & \multicolumn{3}{c|}{{\bf \small PASCAL VOC}} & \multicolumn{3}{c|}{\bf \small COCO} & {\bf \small VOC}      & {\bf \small Cityscapes}                                                                  \\
                                               & { $\text{AP}^b$}                             & { $\text{AP}^b_{50}$}                & { $\text{AP}^b_{75}$} & { $\text{AP}^b$}        & { $\text{AP}^b_{50}$} & {$\text{AP}^b_{75}$} & {mIoU} & {mIoU} \\
            \midrule

            Supervised                         & 50.7                                         & 80.4                                 & 55.1
                                               & 34.0                                         & 54.4                                 & 36.4
                                               & 56.6                                         & 55.7                                                                                                                                                    \\
            Moco v2                            & 52.7                                         & 80.9                                 & 57.6
                                               & 34.0                                         & 53.9                                 & 36.3
                                               & 58.3                                         & 59.1                                                                                                                                                    \\
            BYOL                               & 52.4                                         & 81.1                                 & 57.5
                                               & 34.1                                         & 54.1                                 & 36.8
                                               & 55.7                                         & 55.6                                                                                                                                                    \\
            \midrule
            DetCo                              & 51.3                                         & 79.9                                 & 56.5
                                               & 33.3                                         & 53.5                                 & 35.7
                                               & 56.1                                         & 57.2                                                                                                                                                    \\
            ReSim                              & 53.7                                         & 81.4                                 & 59.6
                                               & 34.4                                         & 54.4                                 & 36.9
                                               & 61.2                                         & 58.1                                                                                                                                                    \\
            SoCo                               & 52.0                                         & 80.0                                 & 56.4
                                               & 33.5                                         & 53.4                                 & 36.1
                                               & 55.2                                         & 56.7                                                                                                                                                    \\
            \midrule
            DenseCL                            & 50.9                                         & 79.9                                 & 55.0
                                               & 33.3                                         & 53.6                                 & 35.8
                                               & 63.0                                         & 58.8                                                                                                                                                    \\
            PixPro                             & 53.5                                         & 80.4                                 & 59.7
                                               & 33.5                                         & 53.1                                 & 36.1
                                               & 60.3                                         & 58.2                                                                                                                                                    \\
            \ours                              & \bf55.1                                      & \bf82.6                              & \bf61.7
                                               & \bf36.0                                      & \bf56.4                              & \bf37.0
                                               & \bf63.4                                      & \bf60.7                                                                                                                                                 \\

            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}



%VOC frozen
\quad
        \begin{tabular}{l c  c  c  c}
                              & \multicolumn{4}{c}{\bf\small Frozen}                                                                               \\
            \toprule
                              & \multicolumn{3}{c}{\bf\small Detection} & \multicolumn{1}{c}{\bf\small Segm}                                       \\
            \cmidrule(lr){2-4} \cmidrule(lr){5-5}
            {}                & {\bf $\text{AP}$}                       & {\bf $\text{AP}_{50}$}             & {\bf $\text{AP}_{75}$} & {\bf mIoU} \\
            \midrule
                              & 32.8                                    & 59.0                               & 31.6                   & -          \\
            %  DenseCL CC & 56.7 & 81.7 & 63.0 & 67.5 \\
            %  \midrule
                              & 50.7                                    & 80.4                               & 55.1                   & 56.6       \\
                              & 52.7                                    & 80.9                               & 57.6                   & 58.3       \\
                              & 52.4                                    & 81.0                               & 57.5                   & 55.7       \\
            \midrule
                              & 51.3                                    & 79.9                               & 56.4                   & 56.1       \\
                              & 53.7                                    & 81.4                               & 59.6                   & 61.2       \\
                              & 52.0                                    & 80.0                               & 56.4                   & 55.2       \\
            \midrule
                              & 50.9                                    & 79.9                               & 55.0                   & 63.0       \\
                              & 53.5                                    & 80.4                               & 59.7                   & 60.3       \\
            \rowcolor{_teal3} & \bf55.1                                 & \bf82.6                            & \bf61.7                & \bf63.4    \\
            \bottomrule
        \end{tabular}
        
        
        

\begin{table}[!htbp]
    \centering
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{l c c c}
                                    & \multicolumn{3}{c}{\bf\small R50-FPN}                                                   \\
            \toprule
            {\bf Method}            & {\bf $\text{AP}$}                     & {\bf $\text{AP}_{50}$} & {\bf $\text{AP}_{75}$} \\
            \midrule
            Scratch                 & 32.8                                  & 50.9                   & 35.3                   \\
            Supervised              & 40.0                                  & 60.1                   & 43.9                   \\
            Moco v2                 & 39.5                                  & 59.3                   & 43.2                   \\
            BYOL                    & 40.6                                  & 60.7                   & 44.1                   \\
            \midrule
            ReSim                   & 40.3                                  & 60.6                   & 44.2                   \\
            SoCo                    & 43.0                                  & 63.3                   & 47.1                   \\
            \midrule
            DetCo                   & 40.1                                  & 61.0                   & 43.9                   \\
            DenseCL                 & 40.3                                  & 59.9                   & 44.3                   \\
            PixPro                  & 41.4                                  & 61.6                   & 45.4                   \\
            \rowcolor{_teal3} \ours & 42.4                                  & 62.8                   & 46.6                   \\
            \bottomrule
        \end{tabular}
        \quad
        \begin{tabular}{l c c c}
                              & \multicolumn{3}{c}{\bf\small RetinaNet-FPN}                                                   \\
            \toprule
                              & {\bf $\text{AP}$}                           & {\bf $\text{AP}_{50}$} & {\bf $\text{AP}_{75}$} \\
            \midrule
                              & -                                           & -                      & -                      \\
                              & 37.7                                        & 57.2                   & 40.4                   \\
                              & 37.3                                        & 56.2                   & 40.4                   \\
                              & 35.4                                        & 54.7                   & 37.4                   \\
            \midrule
                              & 38.6                                        & 57.6                   & 41.6                   \\
                              & -                                           & -                      & -                      \\
            \midrule
                              & 38.4                                        & 57.8                   & 41.2                   \\
                              & 37.6                                        & 56.6                   & 40.2                   \\
                              & 38.7                                        & 57.5                   & 41.6                   \\
            \rowcolor{_teal3} & 40.6                                        & 60.4                   & 43.6                   \\
            \bottomrule
        \end{tabular}
        \quad
        \begin{tabular}{l c c c}
                              & \multicolumn{3}{c}{\bf\small Keypoint-FPN}                                                   \\
            \toprule
                              & {\bf $\text{AP}$}                          & {\bf $\text{AP}_{50}$} & {\bf $\text{AP}_{75}$} \\
            \midrule
                              & -                                          & -                      & -                      \\
                              & 65.7                                       & 87.2                   & 71.5                   \\
                              & 65.9                                       & 86.9                   & 71.6                   \\
                              & 66.3                                       & 87.4                   & 72.4                   \\
            \midrule
                              & 66.6                                       & 87.4                   & 72.8                   \\
                              & -                                          & -                      & -                      \\
            \midrule
                              & -                                          & -                      & -                      \\
                              & 66.2                                       & 87.3                   & 71.9                   \\
                              & 66.6                                       & 87.8                   & 72.8                   \\
            \rowcolor{_teal3} & 67.2                                       & 87.4                   & 73.7                   \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{{\small {\bf COCO object detection} We use 1$\times$ schedule to finetune on COCO \texttt{train2017} and evaluate on \texttt{val2017}.}}
    \label{tab:coco_mask_rcnn}
\end{table}
